Asteroid shape inversion with light curves using deep learning

Asteroid shape inversion using photometric data has been a key area of study in planetary science and astronomical research.However, the current methods for asteroid shape inversion require extensive iterative calculations, making the process time-consuming and prone to becoming stuck in local optima. We directly established a mapping between photometric data and shape distribution through deep neural networks. In addition, we used 3D point clouds to represent asteroid shapes and utilized the deviation between the light curves of non-convex asteroids and their convex hulls to predict the concave areas of non-convex asteroids. We compared the results of different shape models using the Chamfer distance between traditional methods and ours and found that our method performs better, especially when handling special shapes. For the detection of concave areas on the convex hull, the intersection over union (IoU) of our predictions reached 0.89. We further validated this method using observational data from the Lowell Observatory to predict the convex shapes of the asteroids 3337 Milo and 1289 Kuta, and conducted light curve fitting experiments. The experimental results demonstrated the robustness and adaptability of the method

==> ref.tex <==

\begin{thebibliography}{74}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{Achlioptas {et~al.}(2018)Achlioptas, Diamanti, Mitliagkas, \& Guibas}]{achlioptas2018learning}
Achlioptas, P., Diamanti, O., Mitliagkas, I., \& Guibas, L. 2018, in International conference on machine learning, PMLR, 40--49

\bibitem[{{Allworth} {et~al.}(2021){Allworth}, {Windrim}, {Bennett}, \& {Bryson}}]{2021AcAau.181..301A}
{Allworth}, J., {Windrim}, L., {Bennett}, J., \& {Bryson}, M. 2021, Acta Astronautica, 181, 301

\bibitem[{{Bartczak} \& {Dudzi{\'n}ski}(2018)}]{2018MNRAS.473.5050B}
{Bartczak}, P. \& {Dudzi{\'n}ski}, G. 2018, \mnras, 473, 5050

\bibitem[{{Barucci} {et~al.}(1992){Barucci}, {Cellino}, {De Sanctis}, {Fulchignoni}, {Lumme}, {Zappala}, \& {Magnusson}}]{1992A&A...266..385B}
{Barucci}, M.~A., {Cellino}, A., {De Sanctis}, C., {et~al.} 1992, \aap, 266, 385

\bibitem[{Brent(2013)}]{brent2013algorithms}
Brent, R.~P. 2013, Algorithms for minimization without derivatives (Courier Corporation)

\bibitem[{{Carbognani} {et~al.}(2012){Carbognani}, {Tanga}, {Cellino}, {Delbo}, {Mottola}, \& {Marchese}}]{2012P&SS...73...80C}
{Carbognani}, A., {Tanga}, P., {Cellino}, A., {et~al.} 2012, \planss, 73, 80

\bibitem[{{Carry} {et~al.}(2012){Carry}, {Kaasalainen}, {Merline}, {M{\"u}ller}, {Jorda}, {Drummond}, {Berthier}, {O'Rourke}, {{\v{D}}urech}, {K{\"u}ppers}, {Conrad}, {Tamblyn}, {Dumas}, {Sierks}, {Osiris Team}, {A'Hearn}, {Angrilli}, {Barbieri}, {Barucci}, {Bertaux}, {}, {Da Deppo}, {Davidsson}, {Debei}, {De Cecco}, {Fornasier}, {Fulle}, {Groussin}, {Guti{\'e}rrez}, {Ip}, {Keller}, {Koschny}, {Knollenberg}, {Kramm}, {Kuehrt}, {Lamy}, {Lara}, {Lazzarin}, {L{\'o}pez-Moreno}, {Marzari}, {Michalik}, {Naletto}, {Rickman}, {Rodrigo}, {Sabau}, {Thomas}, \& {Wenzel}}]{2012P&SS...66..200C}
{Carry}, B., {Kaasalainen}, M., {Merline}, W.~J., {et~al.} 2012, \planss, 66, 200

\bibitem[{Catmull(1974)}]{catmull1974subdivision}
Catmull, E.~E. 1974, A subdivision algorithm for computer display of curved surfaces (The University of Utah)

\bibitem[{{Cellino} {et~al.}(2024){Cellino}, {Tanga}, {Muinonen}, \& {Mignard}}]{2024A&A...687A.277C}
{Cellino}, A., {Tanga}, P., {Muinonen}, K., \& {Mignard}, F. 2024, \aap, 687, A277

\bibitem[{{Chng} {et~al.}(2022){Chng}, {Sasdelli}, \& {Chin}}]{2022MNRAS.513..311C}
{Chng}, C.-K., {Sasdelli}, M., \& {Chin}, T.-J. 2022, \mnras, 513, 311

\bibitem[{Cohen {et~al.}(2009)Cohen, Huang, Chen, Benesty, Benesty, Chen, Huang, \& Cohen}]{cohen2009pearson}
Cohen, I., Huang, Y., Chen, J., {et~al.} 2009, Noise reduction in speech processing, 1

\bibitem[{Dai {et~al.}(2017)Dai, Ruizhongtai~Qi, \& Nie{\ss}ner}]{dai2017shape}
Dai, A., Ruizhongtai~Qi, C., \& Nie{\ss}ner, M. 2017, in Proceedings of the IEEE conference on computer vision and pattern recognition, 5868--5877

\bibitem[{Daly {et~al.}(2023)Daly, Ernst, Barnouin, Chabot, Rivkin, Cheng, Adams, Agrusa, Abel, Alford, {et~al.}}]{daly2023successful}
Daly, R.~T., Ernst, C.~M., Barnouin, O.~S., {et~al.} 2023, Nature, 616, 443

\bibitem[{Danilova {et~al.}(2022)Danilova, Dvurechensky, Gasnikov, Gorbunov, Guminov, Kamzolov, \& Shibaev}]{danilova2022recent}
Danilova, M., Dvurechensky, P., Gasnikov, A., {et~al.} 2022, in High-Dimensional Optimization and Probability: With a View Towards Data Science (Springer), 79--163

\bibitem[{{Devog{\`e}le} {et~al.}(2015){Devog{\`e}le}, {Rivet}, {Tanga}, {Bendjoya}, {Surdej}, {Bartczak}, \& {Hanus}}]{2015MNRAS.453.2232D}
{Devog{\`e}le}, M., {Rivet}, J.~P., {Tanga}, P., {et~al.} 2015, \mnras, 453, 2232

\bibitem[{Farnham(2013)}]{farnham2013shape}
Farnham, J. 2013, NASA Planetary Data System

\bibitem[{Flavell(2011)}]{flavell2011beginning}
Flavell, L. 2011, Beginning blender: open source 3d modeling, animation, and game design (Apress)

\bibitem[{Groueix {et~al.}(2018)Groueix, Fisher, Kim, Russell, \& Aubry}]{groueix2018papier}
Groueix, T., Fisher, M., Kim, V.~G., Russell, B.~C., \& Aubry, M. 2018, in Proceedings of the IEEE conference on computer vision and pattern recognition, 216--224

\bibitem[{Han {et~al.}(2017)Han, Li, Huang, Kalogerakis, \& Yu}]{han2017high}
Han, X., Li, Z., Huang, H., Kalogerakis, E., \& Yu, Y. 2017, in Proceedings of the IEEE international conference on computer vision, 85--93

\bibitem[{Hao {et~al.}(2023)Hao, Jincheng, Ling, Gengyuan, Sumin, \& Huan}]{hao2023improved}
Hao, H., Jincheng, Y., Ling, Y., {et~al.} 2023, Computers and Electronics in Agriculture, 205, 107560

\bibitem[{{Hapke}(1966)}]{1966AJ.....71..333H}
{Hapke}, B. 1966, \aj, 71, 333

\bibitem[{{Hapke}(1963)}]{1963JGR....68.4571H}
{Hapke}, B.~W. 1963, \jgr, 68, 4571

\bibitem[{{Harris} \& {D'Abramo}(2015)}]{2015Icar..257..302H}
{Harris}, A.~W. \& {D'Abramo}, G. 2015, \icarus, 257, 302

\bibitem[{Hartmann {et~al.}(2024)Hartmann, Ernst, Neumann, \& Alkhatib}]{hartmann2024pointnet}
Hartmann, J., Ernst, D., Neumann, I., \& Alkhatib, H. 2024, Journal of Applied Geodesy

\bibitem[{Huang {et~al.}(2020)Huang, Yu, Xu, Ni, \& Le}]{huang2020pf}
Huang, Z., Yu, Y., Xu, J., Ni, F., \& Le, X. 2020, in Proceedings of the IEEE/CVF conference on computer vision and pattern recognition, 7662--7670

\bibitem[{{Hudson} \& {Ostro}(1998)}]{1998Icar..135..451H}
{Hudson}, R.~S. \& {Ostro}, S.~J. 1998, \icarus, 135, 451

\bibitem[{Hurley \& Rickard(2009)}]{hurley2009comparing}
Hurley, N. \& Rickard, S. 2009, IEEE Transactions on Information Theory, 55, 4723

\bibitem[{{Ivezi{\'c}} {et~al.}(2019){Ivezi{\'c}}, {Kahn}, {Tyson}, {Abel}, {Acosta}, {Allsman}, {Alonso}, {AlSayyad}, {Anderson}, {Andrew}, {Angel}, {Angeli}, {Ansari}, {Antilogus}, {Araujo}, {Armstrong}, {Arndt}, {Astier}, {Aubourg}, {Auza}, {Axelrod}, {Bard}, {Barr}, {Barrau}, {Bartlett}, {Bauer}, {Bauman}, {Baumont}, {Bechtol}, {Bechtol}, {Becker}, {Becla}, {Beldica}, {Bellavia}, {Bianco}, {Biswas}, {Blanc}, {Blazek}, {Blandford}, {Bloom}, {Bogart}, {Bond}, {Booth}, {Borgland}, {Borne}, {Bosch}, {Boutigny}, {Brackett}, {Bradshaw}, {Brandt}, {Brown}, {Bullock}, {Burchat}, {Burke}, {Cagnoli}, {Calabrese}, {Callahan}, {Callen}, {Carlin}, {Carlson}, {Chandrasekharan}, {Charles-Emerson}, {Chesley}, {Cheu}, {Chiang}, {Chiang}, {Chirino}, {Chow}, {Ciardi}, {Claver}, {Cohen-Tanugi}, {Cockrum}, {Coles}, {Connolly}, {Cook}, {Cooray}, {Covey}, {Cribbs}, {Cui}, {Cutri}, {Daly}, {Daniel}, {Daruich}, {Daubard}, {Daues}, {Dawson}, {Delgado}, {Dellapenna}, {de Peyster}, {de Val-Borro}, {Digel}, {Doherty}, {Dubois},
  {Dubois-Felsmann}, {Durech}, {Economou}, {Eifler}, {Eracleous}, {Emmons}, {Fausti Neto}, {Ferguson}, {Figueroa}, {Fisher-Levine}, {Focke}, {Foss}, {Frank}, {Freemon}, {Gangler}, {Gawiser}, {Geary}, {Gee}, {Geha}, {Gessner}, {Gibson}, {Gilmore}, {Glanzman}, {Glick}, {Goldina}, {Goldstein}, {Goodenow}, {Graham}, {Gressler}, {Gris}, {Guy}, {Guyonnet}, {Haller}, {Harris}, {Hascall}, {Haupt}, {Hernandez}, {Herrmann}, {Hileman}, {Hoblitt}, {Hodgson}, {Hogan}, {Howard}, {Huang}, {Huffer}, {Ingraham}, {Innes}, {Jacoby}, {Jain}, {Jammes}, {Jee}, {Jenness}, {Jernigan}, {Jevremovi{\'c}}, {Johns}, {Johnson}, {Johnson}, {Jones}, {Juramy-Gilles}, {Juri{\'c}}, {Kalirai}, {Kallivayalil}, {Kalmbach}, {Kantor}, {Karst}, {Kasliwal}, {Kelly}, {Kessler}, {Kinnison}, {Kirkby}, {Knox}, {Kotov}, {Krabbendam}, {Krughoff}, {Kub{\'a}nek}, {Kuczewski}, {Kulkarni}, {Ku}, {Kurita}, {Lage}, {Lambert}, {Lange}, {Langton}, {Le Guillou}, {Levine}, {Liang}, {Lim}, {Lintott}, {Long}, {Lopez}, {Lotz}, {Lupton}, {Lust}, {MacArthur}, {Mahabal},
  {Mandelbaum}, {Markiewicz}, {Marsh}, {Marshall}, {Marshall}, {May}, {McKercher}, {McQueen}, {Meyers}, {Migliore}, {Miller}, \& {Mills}}]{2019ApJ...873..111I}
{Ivezi{\'c}}, {\v{Z}}., {Kahn}, S.~M., {Tyson}, J.~A., {et~al.} 2019, \apj, 873, 111

\bibitem[{Kaasalainen(2011)}]{kaasalainen2011multimodal}
Kaasalainen, M. 2011, Inverse Problems and Imaging, 5, 37

\bibitem[{{Kaasalainen} {et~al.}(1992{\natexlab{a}}){Kaasalainen}, {Lamberg}, \& {Lumme}}]{1992A&A...259..333K}
{Kaasalainen}, M., {Lamberg}, L., \& {Lumme}, K. 1992{\natexlab{a}}, \aap, 259, 333

\bibitem[{{Kaasalainen} {et~al.}(1992{\natexlab{b}}){Kaasalainen}, {Lamberg}, {Lumme}, \& {Bowell}}]{1992A&A...259..318K}
{Kaasalainen}, M., {Lamberg}, L., {Lumme}, K., \& {Bowell}, E. 1992{\natexlab{b}}, \aap, 259, 318

\bibitem[{{Kaasalainen} \& {Torppa}(2001)}]{2001Icar..153...24K}
{Kaasalainen}, M. \& {Torppa}, J. 2001, \icarus, 153, 24

\bibitem[{{Kaasalainen} {et~al.}(2001){Kaasalainen}, {Torppa}, \& {Muinonen}}]{2001Icar..153...37K}
{Kaasalainen}, M., {Torppa}, J., \& {Muinonen}, K. 2001, \icarus, 153, 37

\bibitem[{{Kaasalainen} \& {Viikinkoski}(2012)}]{2012A&A...543A..97K}
{Kaasalainen}, M. \& {Viikinkoski}, M. 2012, \aap, 543, A97

\bibitem[{{Koehn} {et~al.}(2014){Koehn}, {Bowell}, {Skiff}, {Sanborn}, {McLelland}, {Pravec}, \& {Warner}}]{2014MPBu...41..286K}
{Koehn}, B.~W., {Bowell}, E.~G., {Skiff}, B.~A., {et~al.} 2014, Minor Planet Bulletin, 41, 286

\bibitem[{{Lauretta} {et~al.}(2017){Lauretta}, {Balram-Knutson}, {Beshore}, {Boynton}, {Drouet d'Aubigny}, {DellaGiustina}, {Enos}, {Golish}, {Hergenrother}, {Howell}, {Bennett}, {Morton}, {Nolan}, {Rizk}, {Roper}, {Bartels}, {Bos}, {Dworkin}, {Highsmith}, {Lorenz}, {Lim}, {Mink}, {Moreau}, {Nuth}, {Reuter}, {Simon}, {Bierhaus}, {Bryan}, {Ballouz}, {Barnouin}, {Binzel}, {Bottke}, {Hamilton}, {Walsh}, {Chesley}, {Christensen}, {Clark}, {Connolly}, {Crombie}, {Daly}, {Emery}, {McCoy}, {McMahon}, {Scheeres}, {Messenger}, {Nakamura-Messenger}, {Righter}, \& {Sandford}}]{2017SSRv..212..925L}
{Lauretta}, D.~S., {Balram-Knutson}, S.~S., {Beshore}, E., {et~al.} 2017, \ssr, 212, 925

\bibitem[{{Lee} {et~al.}(2021){Lee}, {{\v{D}}urech}, {Vokrouhlick{\'y}}, {Pravec}, {Moon}, {Ryan}, {Kim}, {Kim}, {Choi}, {Bacci}, {Pollock}, \& {Apitzsch}}]{2021AJ....161..112L}
{Lee}, H.-J., {{\v{D}}urech}, J., {Vokrouhlick{\'y}}, D., {et~al.} 2021, \aj, 161, 112

\bibitem[{{Levison} {et~al.}(2021){Levison}, {Olkin}, {Noll}, {Marchi}, {Bell}, {Bierhaus}, {Binzel}, {Bottke}, {Britt}, {Brown}, {Buie}, {Christensen}, {Emery}, {Grundy}, {Hamilton}, {Howett}, {Mottola}, {P{\"a}tzold}, {Reuter}, {Spencer}, {Statler}, {Stern}, {Sunshine}, {Weaver}, \& {Wong}}]{2021PSJ.....2..171L}
{Levison}, H.~F., {Olkin}, C.~B., {Noll}, K.~S., {et~al.} 2021, PSJ, 2, 171

\bibitem[{{Li} {et~al.}(2015){Li}, {Helfenstein}, {Buratti}, {Takir}, \& {Clark}}]{2015aste.book..129L}
{Li}, J.~Y., {Helfenstein}, P., {Buratti}, B., {Takir}, D., \& {Clark}, B.~E. 2015, in Asteroids IV, ed. P.~{Michel}, F.~E. {DeMeo}, \& W.~F. {Bottke}, 129--150

\bibitem[{{Linares} {et~al.}(2020){Linares}, {Furfaro}, \& {Reddy}}]{2020JAnSc..67.1063L}
{Linares}, R., {Furfaro}, R., \& {Reddy}, V. 2020, Journal of the Astronautical Sciences, 67, 1063

\bibitem[{Lorensen \& Cline(1998)}]{lorensen1998marching}
Lorensen, W.~E. \& Cline, H.~E. 1998, in Seminal graphics: pioneering efforts that shaped the field (ACM Press), 347--353

\bibitem[{Lu {et~al.}(2024)Lu, Zhang, Zhao, Zheng, \& Di}]{lu2024modeling}
Lu, X.-P., Zhang, Y.-X., Zhao, H.-B., Zheng, H., \& Di, K.-C. 2024, The Astrophysical Journal, 961, 154

\bibitem[{Mandikal \& Radhakrishnan(2019)}]{mandikal2019dense}
Mandikal, P. \& Radhakrishnan, V.~B. 2019, in 2019 IEEE Winter Conference on Applications of Computer Vision (WACV), IEEE, 1052--1060

\bibitem[{{Martikainen} {et~al.}(2021){Martikainen}, {Muinonen}, {Penttil{\"a}}, {Cellino}, \& {Wang}}]{2021A&A...649A..98M}
{Martikainen}, J., {Muinonen}, K., {Penttil{\"a}}, A., {Cellino}, A., \& {Wang}, X.~B. 2021, \aap, 649, A98

\bibitem[{{Masoumzadeh} {et~al.}(2015){Masoumzadeh}, {Boehnhardt}, {Li}, \& {Vincent}}]{2015Icar..257..239M}
{Masoumzadeh}, N., {Boehnhardt}, H., {Li}, J.-Y., \& {Vincent}, J.~B. 2015, \icarus, 257, 239

\bibitem[{M{\"o}ller \& Trumbore(2005)}]{moller2005fast}
M{\"o}ller, T. \& Trumbore, B. 2005, in ACM SIGGRAPH 2005 Courses (ACM Press), 7--es

\bibitem[{{Muinonen} \& {Lumme}(2015)}]{2015A&A...584A..23M}
{Muinonen}, K. \& {Lumme}, K. 2015, \aap, 584, A23

\bibitem[{Muinonen {et~al.}(2020)Muinonen, Torppa, Wang, Cellino, \& Penttil{\"a}}]{muinonen2020asteroid}
Muinonen, K., Torppa, J., Wang, X.-B., Cellino, A., \& Penttil{\"a}, A. 2020, Astronomy \& Astrophysics, 642, A138

\bibitem[{{Muinonen} {et~al.}(2022){Muinonen}, {Uvarova}, {Martikainen}, {Penttil{\"a}}, {Cellino}, \& {Wang}}]{2022FrASS...9.1125M}
{Muinonen}, K., {Uvarova}, E., {Martikainen}, J., {et~al.} 2022, Frontiers in Astronomy and Space Sciences, 9, 821125

\bibitem[{{Muinonen} {et~al.}(2015){Muinonen}, {Wilkman}, {Cellino}, {Wang}, \& {Wang}}]{2015P&SS..118..227M}
{Muinonen}, K., {Wilkman}, O., {Cellino}, A., {Wang}, X., \& {Wang}, Y. 2015, \planss, 118, 227

\bibitem[{NASA(2023)}]{nasa}
NASA, P. D.~S. 2023, in https://pds.nasa.gov/datasearch/subscription-service/SS-Release.shtml

\bibitem[{Nguyen {et~al.}(2016)Nguyen, Hua, Tran, Pham, \& Yeung}]{nguyen2016field}
Nguyen, D.~T., Hua, B.-S., Tran, K., Pham, Q.-H., \& Yeung, S.-K. 2016, in Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, 5676--5684

\bibitem[{{Pravec} {et~al.}(2014){Pravec}, {Scheirich}, {{\v{D}}urech}, {Pollock}, {Ku{\v{s}}nir{\'a}k}, {Hornoch}, {Gal{\'a}d}, {Vokrouhlick{\'y}}, {Harris}, {Jehin}, {Manfroid}, {Opitom}, {Gillon}, {Colas}, {Oey}, {Vra{\v{s}}til}, {Reichart}, {Ivarsen}, {Haislip}, \& {LaCluyze}}]{2014Icar..233...48P}
{Pravec}, P., {Scheirich}, P., {{\v{D}}urech}, J., {et~al.} 2014, \icarus, 233, 48

\bibitem[{Qi {et~al.}(2017{\natexlab{a}})Qi, Su, Mo, \& Guibas}]{qi2017pointnet}
Qi, C.~R., Su, H., Mo, K., \& Guibas, L.~J. 2017{\natexlab{a}}, in Proceedings of the IEEE conference on computer vision and pattern recognition, 652--660

\bibitem[{Qi {et~al.}(2017{\natexlab{b}})Qi, Yi, Su, \& Guibas}]{qi2017pointnet++}
Qi, C.~R., Yi, L., Su, H., \& Guibas, L.~J. 2017{\natexlab{b}}, Advances in neural information processing systems, 30

\bibitem[{{Rizos} {et~al.}(2021){Rizos}, {Asensio-Ramos}, {Golish}, {DellaGiustina}, {Licandro}, {de Le{\'o}n}, {Campins}, {Tatsumi}, \& {Popescu}}]{2021arXiv210601363R}
{Rizos}, J.~L., {Asensio-Ramos}, A., {Golish}, D.~R., {et~al.} 2021, arXiv e-prints, arXiv:2106.01363

\bibitem[{{Russell}(1906)}]{1906ApJ....24....1R}
{Russell}, H.~N. 1906, \apj, 24, 1

\bibitem[{{Scheirich} {et~al.}(2010){Scheirich}, {Durech}, {Pravec}, {Kozubal}, {Dantowitz}, {Kaasalainen}, {Betzler}, {Beltrame}, {Muler}, {Birtwhistle}, \& {Kugel}}]{2010M&PS...45.1804S}
{Scheirich}, P., {Durech}, J., {Pravec}, P., {et~al.} 2010, MAPS, 45, 1804

\bibitem[{Sharma {et~al.}(2016)Sharma, Grau, \& Fritz}]{sharma2016vconv}
Sharma, A., Grau, O., \& Fritz, M. 2016, in Computer Vision--ECCV 2016 Workshops: Amsterdam, The Netherlands, October 8-10 and 15-16, 2016, Proceedings, Part III 14, Springer, 236--250

\bibitem[{Stutz \& Geiger(2018)}]{stutz2018learning}
Stutz, D. \& Geiger, A. 2018, in Proceedings of the IEEE conference on computer vision and pattern recognition, 1955--1964

\bibitem[{Tchapmi {et~al.}(2019)Tchapmi, Kosaraju, Rezatofighi, Reid, \& Savarese}]{tchapmi2019topnet}
Tchapmi, L.~P., Kosaraju, V., Rezatofighi, H., Reid, I., \& Savarese, S. 2019, in Proceedings of the IEEE/CVF conference on computer vision and pattern recognition, 383--392

\bibitem[{{{\v{D}}urech}(2002)}]{2002Icar..159..192D}
{{\v{D}}urech}, J. 2002, \icarus, 159, 192

\bibitem[{{{\v{D}}urech} \& {Hanu{\v{s}}}(2023)}]{2023A&A...675A..24D}
{{\v{D}}urech}, J. \& {Hanu{\v{s}}}, J. 2023, \aap, 675, A24

\bibitem[{{{\v{D}}urech} \& {Kaasalainen}(2003)}]{2003A&A...404..709D}
{{\v{D}}urech}, J. \& {Kaasalainen}, M. 2003, \aap, 404, 709

\bibitem[{{{\v{D}}urech} {et~al.}(2010){{\v{D}}urech}, {Sidorin}, \& {Kaasalainen}}]{2010A&A...513A..46D}
{{\v{D}}urech}, J., {Sidorin}, V., \& {Kaasalainen}, M. 2010, \aap, 513, A46

\bibitem[{{{\v{D}}urech} {et~al.}(2020){{\v{D}}urech}, {Tonry}, {Erasmus}, {Denneau}, {Heinze}, {Flewelling}, \& {Van{\v{c}}o}}]{2020A&A...643A..59D}
{{\v{D}}urech}, J., {Tonry}, J., {Erasmus}, N., {et~al.} 2020, \aap, 643, A59

\bibitem[{{Viikinkoski} {et~al.}(2015){Viikinkoski}, {Kaasalainen}, \& {Durech}}]{2015A&A...576A...8V}
{Viikinkoski}, M., {Kaasalainen}, M., \& {Durech}, J. 2015, \aap, 576, A8

\bibitem[{Wang {et~al.}(2019)Wang, Sun, Liu, Sarma, Bronstein, \& Solomon}]{wang2019dynamic}
Wang, Y., Sun, Y., Liu, Z., {et~al.} 2019, ACM Transactions on Graphics (tog), 38, 1

\bibitem[{{Watanabe} {et~al.}(2019){Watanabe}, {Hirabayashi}, {Hirata}, {Hirata}, {Noguchi}, {Shimaki}, {Ikeda}, {Tatsumi}, {Yoshikawa}, {Kikuchi}, {Yabuta}, {Nakamura}, {Tachibana}, {Ishihara}, {Morota}, {Kitazato}, {Sakatani}, {Matsumoto}, {Wada}, {Senshu}, {Honda}, {Michikami}, {Takeuchi}, {Kouyama}, {Honda}, {Kameda}, {Fuse}, {Miyamoto}, {Komatsu}, {Sugita}, {Okada}, {Namiki}, {Arakawa}, {Ishiguro}, {Abe}, {Gaskell}, {Palmer}, {Barnouin}, {Michel}, {French}, {McMahon}, {Scheeres}, {Abell}, {Yamamoto}, {Tanaka}, {Shirai}, {Matsuoka}, {Yamada}, {Yokota}, {Suzuki}, {Yoshioka}, {Cho}, {Tanaka}, {Nishikawa}, {Sugiyama}, {Kikuchi}, {Hemmi}, {Yamaguchi}, {Ogawa}, {Ono}, {Mimasu}, {Yoshikawa}, {Takahashi}, {Takei}, {Fujii}, {Hirose}, {Iwata}, {Hayakawa}, {Hosoda}, {Mori}, {Sawada}, {Shimada}, {Soldini}, {Yano}, {Tsukizaki}, {Ozaki}, {Iijima}, {Ogawa}, {Fujimoto}, {Ho}, {Moussi}, {Jaumann}, {Bibring}, {Krause}, {Terui}, {Saiki}, {Nakazawa}, \& {Tsuda}}]{2019Sci...364..268W}
{Watanabe}, S., {Hirabayashi}, M., {Hirata}, N., {et~al.} 2019, Science, 364, 268

\bibitem[{Yu {et~al.}(2021)Yu, Rao, Wang, Liu, Lu, \& Zhou}]{yu2021pointr}
Yu, X., Rao, Y., Wang, Z., {et~al.} 2021, in Proceedings of the IEEE/CVF international conference on computer vision, 12498--12507

\bibitem[{Yuan {et~al.}(2018)Yuan, Khot, Held, Mertz, \& Hebert}]{yuan2018pcn}
Yuan, W., Khot, T., Held, D., Mertz, C., \& Hebert, M. 2018, in 2018 international conference on 3D vision (3DV), IEEE, 728--737

\bibitem[{{Zhang} {et~al.}(2024){Zhang}, {Li}, {Zhang}, {Yan}, {Zhang}, {Vernazza}, {Cloutis}, {Hiroi}, {Granvik}, {Zhang}, \& {Lin}}]{2024LPICo3040.1845Z}
{Zhang}, P.~F., {Li}, Y., {Zhang}, G.~Z., {et~al.} 2024, in LPI Contributions, Vol. 3040, 55th Lunar and Planetary Science Conference, 1845

\bibitem[{Zhou {et~al.}(2022)Zhou, Cao, Chu, Zhu, Lu, Tai, \& Wang}]{zhou2022seedformer}
Zhou, H., Cao, Y., Chu, W., {et~al.} 2022, in European conference on computer vision, Springer, 416--432

\bibitem[{Zuber {et~al.}(2000)Zuber, Smith, Cheng, Garvin, Aharonson, Cole, Dunn, Guo, Lemoine, Neumann, {et~al.}}]{zuber2000shape}
Zuber, M.~T., Smith, D.~E., Cheng, A.~F., {et~al.} 2000, Science, 289, 2097

\end{thebibliography}

